DeepStyle: User Style Embedding for Authorship Attribution of Short Texts

Authorship attribution (AA), which is the task of finding the owner of a given text, is an important and widely studied research topic with many applications. Recent works have shown that deep learning methods could achieve significant accuracy improvement for the AA task. Nevertheless, most of these proposed methods represent user posts using a single type of feature (e.g., word bi-grams) and adopt a text classification approach to address the task. Furthermore, these methods offer very limited explainability of the AA results. In this paper, we address these limitations by proposing DeepStyle, a novel embedding-based framework that learns the representations of users' salient writing styles. We conduct extensive experiments on two real-world datasets from Twitter and Weibo. Our experiment results show that DeepStyle outperforms the state-of-the-art baselines on the AA task.

==> APWEB20 - DeepStyle (Cam-Ready)/conclusion.tex <==
In this paper, we proposed a novel embedding-based framework call \textsf{DeepStyle}, which utilized multiple feature types to learns the embedding representation of the user's writing style for authorship attribution (AA). We evaluated \textsf{DeepStyle} using publicly available real-world datasets, and our extensive experiments have shown that \textsf{DeepStyle} is language-agnostic and outperforms the baselines in different experimental settings. For future works, we will like to consider the evolution of the user's writing style by modeling the time-series aspect of the user's posts and consider other better forms of visualizations to explain the user's writing style. 

%We have also empirically analyzed the learned user style embeddings and demonstrated \textsf{DeepStyle}'s ability to capture the salient features from the user's posts, which can help to define the user's writing style. This helps to provide some form of explainability to AA methods.

==> APWEB20 - DeepStyle (Cam-Ready)/experiment.tex <==
%In this section, we first discuss the datasets and baselines used in our experiments. Next, we discuss the results of our authorship attribution experiments. We also conduct further analysis to examine the learned user style embedding and salient features learned from our proposed framework.

\subsection{Experiment Setup}
\textbf{Datasets.} We conducted our experiments on two publicly available datasets, namely Weibo\footnote{https://hub.hku.hk/cris/dataset/dataset107483} and Twitter \cite{schwartz2013authorship}. The Twitter dataset is widely used in AA research \cite{schwartz2013authorship,shrestha2017convolutional}, while the Weibo dataset, which consists of short Chinese texts, demonstrates the language-agnostic nature of our model. The Twitter dataset contains tweets from 7,026 users, while the Weibo dataset contains posts from 9,819 users. In both datasets, each user has about 1000 posts.

\textbf{Baselines.} For evaluation, we compare our proposed \textsf{DeepStyle} model with the following state-of-the-art baselines:
\begin{itemize}
    \item \textbf{ToS}: Based on \cite{sari2018topic}'s work, ToS method derives content and style-based features from the users' posts to train a Logistic Regression classifier.  
    \item \textbf{CNN}: Following the studies in \cite{shrestha2017convolutional,DBLP:journals/corr/RuderGB16c}, we train a CNN model each on character features (called CNN-1), bigram features (called CNN-2), and word features ( called CNN-W).
    \item \textbf{LSTM}: Long-Short Term Memory (LSTM) model has also been implemented as a baseline in previous study \cite{shrestha2017convolutional} and the model has been  successfully used for text classification \cite{liu2016recurrent}. We train an LSTM at the character level (LSTM-1),  bigram level  (LSTM-2), and word (LSTM-W) level.
\end{itemize}
All the parameters of baselines are empirically set to yield optimal results. 

%Besides the baselines, we also test several variants of the \textsf{DeepStyle} framework:
%\begin{itemize}
%    \item \textbf{DS-CNN}: We use multiple CNNs in our post embedding module to learn the post embeddings from user posts. We also explore three types of aggregators (i.e., mean, max, and capsule) to aggregate post embeddings to form the user style embeddings.     
%    \item \textbf{DS-LSTM}: We replace the CNN with LSTM in our post embedding module to extract various style features from the users' posts to learn the post embeddings. We use capsule aggregator to aggregate the posts embeddings to form the user style embeddings.
%\end{itemize}

% \textbf{Training and Testing Set.} In our experiments, we adopt an 80-20 split, where 80\% of each user's posts are used for training with the remaining 20\% used for testing.  Note that for different experiments, we may vary the number of user posts used to illustrate the robustness of our model. However, the train-test ratio remains the same. 

% \textbf{Evaluation Metrics.} For the evaluation metric, we use \textit{Precision at top k (P@$k$)}, where a prediction is considered as correct when the top $k$ ranked users predicted by a model for a given test query post contains the ground truth author. Also, five-fold cross-validation is used in our experiments, and the average results of the five folds are reported.

\subsection{Experiment Results}
Table \ref{tbl:resultspostK} shows the experiment results on Twitter and Weibo datasets. In this experiment, we use 100 posts from each user for training and test on 20 posts from each user. All users on Twitter and Weibo are used in this experiment. Note that the \textsf{DeepStyle} model in this experiment is configured with \textit{Capsule} as the feature fusion function to combine the various latent representations of a post and we select \textit{Mean} as the aggregator to combine the users' post embeddings into final user style embeddings. The same \textsf{DeepStyle} setting is used for the results reported in Tables~\ref{tbl:results} and \ref{tbl:resultspost}. From the results, we observe that \textsf{DeepStyle} outperforms the state-of-the-art baselines for different $k$ values using the $P@k$ measure. The improvements of \textsf{DeepStyle} over the best baselines (i.e., CNN-1 and CNN-2) are significant at 0.01 level using paired t-test. Similar to the previous study \cite{shrestha2017convolutional}, we observe that the CNN models outperform the LSTM models in both datasets. More interestingly, CNN-2 performs better than CNN-1 for the Twitter dataset, while CNN-1 outperforms CNN-2 for the Weibo dataset. This observation could be attributed to the difference in languages; Chinese characters may encode more semantics or definitive user styles. Hence, the Chinese character unigrams can yield better results.  \textsf{DeepStyle}, which utilizes multi-style post representations, outperforms all state-of-the-art baselines in both English (i.e., Twitter) and Chinese (i.e., Weibo) datasets.

\begin{table}[t]
\centering
\caption{P@k of various baselines and \textsf{DeepStyle} on Twitter and Weibo datasets. We vary $k = [1, 10, 50, 100]$. The improvement of \textsf{DeepStyle} over the best baselines (i.e., CNN-1) is significant at 0.01 level using paired t-test.}
\label{tbl:resultspostK}
\begin{tabular}{|l|cccc|cccc|}
\hline
 & \multicolumn{4}{c|}{\textbf{Twitter}}&\multicolumn{4}{c|}{\textbf{Weibo}}\\
{\textbf{Method}} & {\textbf{P@1}} & {\textbf{P@10}} & {\textbf{P@50}} & {\textbf{P@100}}& {\textbf{P@1}} & {\textbf{P@10}} & {\textbf{P@50}} & {\textbf{P@100}} \\
\hline \hline
ToS \cite{sari2018topic}  &9.8 &20.4 &32.2 &43.0 &12.1  &25.9  &38.6  &48.3  \\\hline
CNN-1 \cite{shrestha2017convolutional,DBLP:journals/corr/RuderGB16c} &18.7 &30.7 &43.1 &49.9 &22.0  &35.2  &48.4 &55.9  \\
CNN-2 \cite{shrestha2017convolutional} &20.1 &33.7 &47.6 &55.3 &17.5  &29.7  &41.3  &51.3  \\
CNN-W \cite{shrestha2017convolutional,DBLP:journals/corr/RuderGB16c} &16.4 &27.1 &37.6 &44.0 &21.0 &36.5  &48.6  &54.8  \\\hline
LSTM-1 &15.3 &25.6 &35.9 &42.0 &19.0  &33.6  &48.1 &55.5  \\
LSTM-2 \cite{shrestha2017convolutional} &15.5 &28.0 &40.9 &48.6 &15.8 &31.5  &43.5  &49.8  \\
LSTM-W &11.7 &23.7 &41.2 &48.1 &18.7  &34.1  &48.0  &55.2  \\\hline
DeepStyle &\textbf{21.4} &\textbf{37.1} &\textbf{51.5} &\textbf{59.2} & \textbf{23.9} & \textbf{38.1} & \textbf{51.6} &\textbf{58.9} \\
% DS-LSTM &0.513 &0.434 &0.359 &0.340 &  &  &  &  \\
\hline
\end{tabular}
\end{table}

\textbf{Varying number of users and posts.} Similar to previous studies \cite{shrestha2017convolutional,schwartz2013authorship}, we also want to explore how \textsf{DeepStyle} performs when the AA problem becomes more difficult, i.e., when the number of users increases or when the number of tweets per author is reduced. Table~\ref{tbl:results} shows the $P@1$ of DeepStyle and various baselines varying the number of users in Twitter and Weibo from 50 to all users. For this experiment, we use 100 posts from each user for training and test on 20 posts from each user. We note that although the precision decreases with the increasing number of users, \textsf{DeepStyle} is able to outperform state-of-the-art baselines consistently. Even in the worse case of all users, i.e., over 7,000 and 9,000 Twitter and Weibo users respectively, \textsf{DeepStyle} is still able to outperform the best baselines and the improvements over the best baselines are significant at 0.01 level using paired t-test.

Besides varying the number of users, we also conducted experiments to evaluate the models' performance with different amounts of training data. Table~\ref{tbl:resultspost} shows the results of the models trained with a different number of posts per user for 50 randomly selected Twitter and Weibo users. We observe the $P@1$ of various models drops as we reduce the number of posts. However, \textsf{DeepStyle} still consistently outperforms the baselines even with reduced training data.

\begin{table*}[t]
\centering
\caption{P@1 for \textsf{DeepStyle} and baselines on varying number of users in Twitter and Weibo. }
\label{tbl:results}
\begin{tabular}{|l|ccccc|ccccc|}
\hline
 & \multicolumn{5}{c|}{\textbf{\#Twitter Users}} & \multicolumn{5}{c|}{\textbf{\#Weibo Users}} \\
{\textbf{Method}} & {\textbf{50}} & {\textbf{100}} & {\textbf{500}} & {\textbf{5000}} & {\textbf{All}} & {\textbf{50}} & {\textbf{100}} & {\textbf{500}} & {\textbf{5000}} & {\textbf{All}} \\\hline \hline
ToS \cite{sari2018topic} &48.3 &31.2 &22.0 &15.7 &9.8 &50.5 &39.5 &22.2 &16.0 &12.1 \\\hline
CNN-1 \cite{shrestha2017convolutional,DBLP:journals/corr/RuderGB16c} &60.9 &47.1 &35.6 &23.1 &18.7 &61.3 &52.6 &38.8 &25.1 &22.0 \\
CNN-2 \cite{shrestha2017convolutional} &59.3 &46.7 &36.5 &24.6 &20.1 &47.6 &42.4 &30.4 &18.7 &17.5 \\
CNN-W \cite{shrestha2017convolutional,DBLP:journals/corr/RuderGB16c} &50.0 &37.1 &28.4 &17.7 &16.4 &56.8 &48.3 &36.2 &23.8 &21.0 \\\hline
LSTM-1 &40.3 &29.6 &27.3 &16.1 &15.3 &37.5 &32.5 &30.9 &20.1 &19.0 \\
LSTM-2 \cite{shrestha2017convolutional} &45.1 &34.5 &25.2 &16.5 &15.5 &28.1 &26.4 &19.6 &16.8 &15.8 \\
LSTM-W &35.0 &22.8 &19.3 &12.0 &11.7 &35.0 &33.4 &28.8 &19.8 &18.7 \\\hline 
%DS-CNN-Max  &0.631 &0.442 &0.329 &0.201 &0.152 &0.631 &0.512 &0.382 &0.222 &0.173 \\
%DS-CNN-Capsule &0.642 &0.510 &\textbf{0.380} &0.252 &0.214 &0.650 &0.563 &0.426 &0.277 &0.237 \\
DeepStyle & \textbf{64.8} & \textbf{51.2} & \textbf{37.9} & \textbf{25.5} & \textbf{21.4} & \textbf{65.2} & \textbf{56.6} & \textbf{42.8} &\textbf{27.9} &\textbf{23.9} \\
% DS-LSTM &0.416 &0.268 &0.195 &0.133 &0.125 &0.378 &0.301 &0.233 &0.189 &0.161 \\
\hline
\end{tabular}
\end{table*}
 
%Note that we use Capsule as the fusion function to combine the various latent representations of a post, and we report the results for three types of aggregators used to form the user style embeddings. The comparison of various fusion functions is discussed in Table \ref{tbl:resultsfusion}. From the results, we observed that DS-CNN-Mean outperforms the baselines and other \textsf{DeepStyle} models. Similar to previous studies \cite{shrestha2017convolutional,schwartz2013authorship}, we also observe that as the number of authors increases, the performances of all AA methods drop.  This is due to the problem becoming more difficult. However, even in the worse case of all users, DS-CNN-Mean still outperforms the other baselines in the Twitter and Weibo datasets.

%\vspace{12px}
\begin{table}[t]
\centering
\caption{P@1 for \textsf{DeepStyle} and baselines on varying number of posts for 50 Twitter and Weibo users.}
\label{tbl:resultspost}
\begin{tabular}{|l|cccc|cccc|}
\hline
 & \multicolumn{4}{c|}{\textbf{Twitter\#posts}}&\multicolumn{4}{c|}{\textbf{Weibo\#posts}}\\
{\textbf{Method}} & {\textbf{500}} & {\textbf{200}} & {\textbf{100}} & {\textbf{50}}& {\textbf{500}} & {\textbf{200}} & {\textbf{100}} & {\textbf{50}} \\
\hline \hline
ToS \cite{sari2018topic} &47.4 &45.1 &40.5 &36.2 & 49.2 & 44.9 & 40.8 & 34.7 \\\hline
CNN-1 \cite{shrestha2017convolutional,DBLP:journals/corr/RuderGB16c} &59.6 &56.0 &51.7 &49.3 & 60.5 & 56.7 & 52.2 & 49.1 \\
CNN-2 \cite{shrestha2017convolutional} &61.7 &54.1 &48.4 &44.4 & 59.4 & 56.3 & 51.8 & 47.5 \\
CNN-W \cite{shrestha2017convolutional,DBLP:journals/corr/RuderGB16c} &52.1 &48.0 &43.3 &40.2 & 58.0 & 53.1 & 47.9 & 44.2 \\\hline
LSTM-1 &55.7 &49.5 &39.8 &32.9 &54.7 &48.7 &37.6  &32.0  \\
LSTM-2 \cite{shrestha2017convolutional} &53.2 &39.4 &34.2 &30.4 &51.0  &42.4 &35.5 &31.4  \\
LSTM-W &47.6 &41.5 &35.2 &30.5 &52.8  &41.9  &36.1  &31.2  \\\hline
DeepStyle &\textbf{62.8} &\textbf{58.7} &\textbf{56.3} &\textbf{50.9} & \textbf{62.5} & \textbf{58.2} & \textbf{56.1} &\textbf{51.1} \\
% DS-LSTM &0.513 &0.434 &0.359 &0.340 &  &  &  &  \\
\hline
\end{tabular}
\end{table}
%\vspace{-15px}

% \textbf{Ablation studies.} In this evaluation, we perform ablation study to investigate the effects of different post representations and the impact of two important components in the \textsf{DeepStyle} model, namely, (i) fusion method to combine the multi-style post representations, and (ii) aggregator module to aggregate a user's multiple post embeddings to form the user style embedding. In the experiments for ablation study, we trained using 100 posts per user, and randomly selected 50 Twitter and Weibo users for reporting results. Table~\ref{tbl:resultablation} shows the results of \textsf{DeepStyle} model using the different combinations of post style features. We note that the setting using all features performed the best in both datasets, suggesting that each type of post styles features can contribute to the AA task. 

% \begin{table}[t]
% \centering
% \caption{P@1 of \textsf{DeepStyle} using different post style features.}
% \label{tbl:resultablation}
% \begin{tabular}{|c|c|c|}
% \hline
% %& \multicolumn{1}{c|}{\textbf{Twitter}}&\multicolumn{1}{c|}{\textbf{Weibo}}\\
% \textbf{Model} & \textbf{Twitter P@1} & \textbf{Weibo P@1}\\\hline \hline
% All Features & \textbf{64.8} & \textbf{65.2} \\
% Word + Character + Bi-gram  & 63.9 & 64.4\\
% Character + Bi-gram &  62.8 & 63.4\\
% Bi-gram & 61.7 & 62.1\\
% \hline
% \end{tabular}
% \end{table}

% \begin{table}[t]
% \centering
% \caption{Comparison of various fusion methods used in post embedding module.}
% \label{tbl:resultsfusion}
% \begin{tabular}{|c|c|c|}
% \hline
% %& \multicolumn{1}{c|}{\textbf{Twitter}}&\multicolumn{1}{c|}{\textbf{Weibo}}\\
% \textbf{Fusion Method} & \textbf{Twitter P@1} & \textbf{Weibo P@1} \\\hline \hline
% Capsule & \textbf{64.8} & \textbf{65.2} \\
% Mean & 63.6 & 64.1 \\
% Max &  63.1 &  62.8\\
% Attention & 63.3 & 64.0 \\
% MLP &  62.6 & 63.4 \\
% \hline
% \end{tabular}
% \end{table}

% \begin{table}[t]
% \centering
% \caption{Comparison of aggregators used in user style aggregation module.}
% \label{tbl:resultsaggregate}
% \begin{tabular}{|c|c|c|}
% \hline
% %& \multicolumn{1}{c|}{\textbf{Twitter}}&\multicolumn{1}{c|}{\textbf{Weibo}}\\
% \textbf{Aggregator} & \textbf{Twitter P@1} & \textbf{Weibo P@1} \\\hline \hline
% Capsule & 64.2 & 65.0 \\
% Mean & \textbf{64.8} & \textbf{65.2} \\
% Max &  63.1 &  63.1\\
% \hline
% \end{tabular}
% \end{table}

% Table~\ref{tbl:resultsfusion} shows the comparison of \textsf{DeepStyle} model implemented with various fusion methods used to combine the multi-style post representations. In this experiment, we select \textit{Mean} as the aggregator to combine the users' post embeddings into final user style embeddings. The table shows that the Capsule method outperforms the other fusion methods to combine multi-style post representations effectively. Table~\ref{tbl:resultsaggregate} shows the comparison of \textsf{DeepStyle} model implemented with various aggregators to combine the users' post embeddings into the final user style embedding. In this experiment, we use \textit{Capsule} as the fusion method to combine the multi-style post representations. We observe that the \textbf{Mean} aggregator outperforms the other  aggregators, suggesting that the styles of posts published by a user are quite similar, and the user's posts are close to one another in the post embedding space.



%\begin{table}[t]
%\centering
%\caption{Comparison of various types of user post embedding aggregators method used in user style embedding module. Results are based on training 100 posts per user for 50 users in Twitter.}
%\label{tbl:resultsggregator}
%\begin{tabular}{|c|c|c|}
%\hline
%%& \multicolumn{1}{c|}{\textbf{Twitter}}&\multicolumn{1}{c|}{\textbf{Weibo}}\\
%\textbf{Aggregator} & \textbf{Twitter P@1} & \textbf{Weibo P@1} \\\hline \hline
%Mean & \textbf{0.648} & \textbf{0.652} \\
%Max &  0.631 &  0.631\\
%Capsule & 0.642 &  0.650\\
%\hline
%\end{tabular}
%\end{table}


% \subsection{User Style Embeddings Analysis}
% Figure~\ref{fig:embeddings} shows the visualizations of the learned post embeddings of 10 Twitter users over the training epochs using t-SNE \cite{maaten2008visualizing}. We observe that over the training epochs, the post embeddings begin to cluster such that the posts of a user would move closer to one another in the embedding space while the posts of different users are ``pushed apart''. Consequently, when we aggregate the post embeddings of individual users to generate the user style embeddings, the embeddings between different users will also be pushed further apart in the embedding space over time. The epoch transitions of the post embeddings demonstrate \textsf{DeepSyle}'s capabilities to learn latent features that differentiate posts of different users, and this important characteristics fundamentally enables us to apply \textsf{DeepStyles} to the AA problem. 


% \begin{figure*}[t] 
% 	\centering
% 	\setlength{\tabcolsep}{0pt} % Default value: 6pt
% 	\renewcommand{\arraystretch}{0} % Default value: 1
% 	\begin{tabular}{cccc}
% 		\includegraphics[scale = 0.15]{post_epoch0.eps} &   
%         \includegraphics[scale = 0.15]{post_epoch1.eps} &
%         \includegraphics[scale = 0.15]{post_epoch5.eps} &
%         \includegraphics[scale = 0.15]{post_epoch10.eps} \\
% %		\includegraphics[scale = 0.15]{user_epoch0.eps} &   
% %        \includegraphics[scale = 0.15]{user_epoch1.eps} &
% %        \includegraphics[scale = 0.15]{user_epoch5.eps} &
% %        \includegraphics[scale = 0.15]{user_epoch10.eps} \\
% 	\end{tabular}
% 	\caption{Temporal transition of the post embeddings of 10 Twitter users.}
% 	\label{fig:embeddings}
% \end{figure*}


% \subsection{Sailent Feature Analysis}
% To analyze how our \textsf{DeepStyle} models the user's writing style, we examine the importance of different feature types and the most salient sections of a single post in different input representations. Figure~\ref{fig:casestudy}(a) shows two Twitter posts from the same user represented using different types of input features, i.e., word, character, bi-gram, and POS tag. The weights of the various features types learned using the capsule fusion method in \textsf{DeepStyle} are visualized in different shades of yellow; the darker the shade, the higher the weight assigned to the feature type used to represent the final post embedding. For the first two posts belonging to the same user, we observe that the character and bi-gram input feature types are more important, and given larger weights. Similar observations are made for two Weibo posts from another user in Figure~\ref{fig:casestudy}(b). Empirically, we also observe the varying importance of the different input features across posts and users. The \textsf{DeepStyle} model can handle the dynamics in feature type importance and learn the underlying representation that best represents each user's writing style.

% \begin{figure}[t] 
%     \centering
%     \setlength{\tabcolsep}{0pt} % Default value: 6pt
%     \renewcommand{\arraystretch}{0} % Default value: 1
%     \begin{tabular}{c}
%         \includegraphics[scale = 0.8]{viz_twitter.pdf} \\ Fig. A\\   
%         \includegraphics[scale = 0.8]{viz_weibo.pdf} \\ Fig. B\\ 
%     \end{tabular}
%     \caption{Visualized saliency scores of (A) Twitter and (B) Weibo posts from same user}
%     \label{fig:casestudy}
% \end{figure}


% Besides understanding the importance of different types of feature input, we examine which sections of a post's input feature representations are most salient in defining the user's writing style. We adopt the saliency score defined by \cite{li2016visualizing} to measure the saliency of input features, and the saliency score was also used in other AA works \cite{shrestha2017convolutional,Boenninghoff2019}. The score indicates how sensitive a model is to the changes in the embedding input, i.e., in our case, how much a specific word, character, n-gram, or POS tag, contributes to the final decision. We visualize the computed saliency scores in Figure~\ref{fig:casestudy} such that the more salient that section of the posts' input feature representation is, the darker is its shade of red. For the first two Twitter posts in Figure~\ref{fig:casestudy}(a), we observe that the user tends to begin a post with nouns and use the function word, ``(not)''. From the salient sections in character and bi-gram features, we also observe that the usage of the words containing the bi-gram  ``ll'' may also be indicative of the user's writing style. On the other hand, the indicative characters highlighted for the Weibo posts (Figure ~\ref{fig:casestudy}(b)) tend to be topical; many of the salient Chinese characters are related to the ``mountain hiking'' topic. Thus, the interests in mountain hiking and frequent use of Chinese characters related to the topic may be indicative of the user's posts. This interesting observation of indicative topical characters also illustrates the rich information encoded in Chinese characters. Essentially, \textsf{DeepStyle} offers a more holistic perspective to how users express themselves in short-text, and it enables us to perform more in-depth studies on the various input features representations of users' post to better profile users' writing styles.  


==> APWEB20 - DeepStyle (Cam-Ready)/introduction.tex <==
\textbf{Motivation.} Authorship attribution (AA), the task of finding the owner of a given text, plays a vital role in many applications. Particularly in the context of social media, AA is crucial in tackling the growing problem of online falsehood, vicious sock-puppets, and evidence gathering in forensic investigations. Although the AA task has been widely studied and many features have been explored \cite{layton2010authorship,koppel2014determining,sapkota2015not,schwartz2013authorship,sundararajan2018represents,sari2018topic}, the traditional document-based methods did not perform well on the social media posts as they tend to be shorter and less former \cite{koppel2014determining,shrestha2017convolutional}. 

To overcome the short-text challenge, several previous AA works have aggregated multiple social media posts of the same user into a single long document before training a classifier to predict the author labels using the long document features, \cite{ding2017learning,layton2010authorship}. Such an approach is, however, not effective in handling AA for individual query or a single social media post, which is necessary for some applications, e.g., detecting if two social media posts sharing a rumor originate from the same person. In a recent study, \cite{shrestha2017convolutional} used n-grams of individual Twitter posts to train a Convolutional Neural Network (CNN) model for AA. While CNN and other deep learning models can achieve improved accuracy for the AA task, they still have several limitations. Firstly, the existing models only utilized single input feature types (e.g., bi-gram) to represent the post. Such approaches neglect the rich types of features which had been explored in previous studies to overcome data sparsity in representing the user's writing styles from short text \cite{sari2018topic}. Secondly, the deep learning approach usually offers limited explainability on how some factors contribute to good (or bad) AA results as the models themselves are black boxes.

\textbf{Research Objectives.} In this paper, we address the limitations in existing methods and propose \textsf{DeepStyle}\footnote{Code implementation: https://gitlab.com/bottle\_shop/snlg/style/deepstyle}, an embedding-based framework specifically designed to learn the user style representations using deep learning. The key idea behind \textsf{DeepStyle} is to extract salient features from the users' social media posts. At the high level, our proposed \textsf{DeepStyle} is divided into two parts.  The first part learns a multi-view representation of a user's posts using deep neural networks over different types of features. Unlike existing deep learning AA methods which use Cross-Entropy loss as objective function, we adopt Triplet loss  \cite{cheng2016person} to learn the post embeddings such that posts that belong to the same user should be close to one another in the post embedding space, while posts from different users will be pushed further away from one another. The second part involves the use of an aggregation function to combine the post embeddings of a single user into the user's style embedding. The underlying intuition is that the style embeddings of different users should be far apart from one another in the embedding space, thereby distinguishing the users' writing styles. Finally, the learned user style embeddings are used to perform the AA task. 

There are benefits to learning user style embeddings. Firstly, the user style embedding allows us to perform AA in both unsupervised (i.e., finding the most similar user in the embedding space for a given query post) and supervised (i.e., as input to a classifier) settings. Secondly, the visualization of user style embedding enables us to gain an understanding of the feature differences and relationships between user writing styles. Lastly, beyond AA, the user style embedding can also be used for other forensic investigations such as clone \cite{xiao2015detecting} or sock-puppet account detection \cite{bu2013sock} by finding the nearest neighbors in the embedding space,i.e., user accounts who share most similar writing style.

\textbf{Contributions.}
Our main contributions in this work consist of the following.
\begin{itemize}
    \item We propose a novel embedding-based framework called \textsf{DeepStyle}, which utilizes multi-view representations of a user's post and Triplet loss objective functions to learn users' writing style for AA.
    \item Using \textsf{DeepStyle}, we manage to learn the latent representation of users' writing style. To the best of our knowledge, this is the first work that embeds user's writing style for AA. 
    \item We conduct extensive experiments on two real-world datasets from Twitter and Weibo. The experiment results show that \textsf{DeepStyle} consistently outperforms state-of-the-art methods regardless of the text's languages. 
    %\item We conduct empirical analyses on the trained user style embedding and provide insights into the salient features that best defines a user's writing style.
\end{itemize}


==> APWEB20 - DeepStyle (Cam-Ready)/model.tex <==
%In this section, we first define the AA problem. We then present our proposed framework, \textsf{DeepStyle}.  The \textsf{DeepStyle} framework utilizes deep learning methods to learn a representation of user writing styles which can be subsequently used for AA task.  

%. The whole framework consists of two modules. The first component, as illustrated in Figure \ref{fig:framework_post_learning}, namely \textit{post embedding module}, learns the representation of user's posts using deep neural networks over various types of features derived from user's posts. To get a single user's style embedding, the second component, called as \textit{user embedding module}, uses an aggregation module without learning to aggregate the post representations of this user taking advantage of learned \textit{post embedding module}.

%In the following, we first formulate authorship attribution (AA) problem. Then, we present the design of \textit{post embedding module} and its optimization. At last, we introduce three sorts of aggregation methods to obtain user representation. 

\subsection{Authorship Attribution Problem}
%Before introducing the two modules of our framework, we first formulate the authorship attribution problems. 
Let $U$ be a set of users in a social media platform, $U=\{u_1,u_2,...,u_N\}$, where $N$ is the total number of users in the platform. Each user $u$ has a set of posts, $P_{u}=\{p_{u,1},p_{u,1},...,p_{u,M_u}\}$, where $M_u$ is the number of posts belong to user $u$. Given $U$, $P_u$, and a query post $q$, we aim to predict the most likely author of $q$.

Traditionally, a classifier will be trained using the known posts of all users to predict the most plausible author of $q$. In this paper, we adopt a different approach by first learning post embeddings of a user $u$ with $M_u$ posts.  The symbol $e_{u,i}$ denotes the post representation of post $p_{u,i}$. The learned post embeddings $E_u = \{e_{u,1}, \cdots, e_{u,M_u}\}$ will then be aggregated to form the user style embedding $s_u$.  Finally, we compute for each user $u$ the cosine similarity between the query post embedding $e^q$ and $s_u$, denoted by $cos(e^q,s_u)$. Our model predicts the top similar user to be most plausible author of query post $q$.  In the following, we elaborate both the \textit{post embedding} and \textit{user style aggregation} modules.

%We formulate AA problem as follows. For social platforms such as Twitter and Weibo, there is a set of $M$ users $U=\{u_1, u_2, ..., u_M\}$. For certain user $u_i$, there are a series of $N$ posts $P_{u_i}=\{p_{u_i,1}, p_{u_i,2}, ..., p_{u_i,N}\}$ and each post contains $T$ words $W_{u_i,p_j}=\{w_{i,j,1}, w_{i,j,2}, ..., w_{i,j,T}\}$. Given all known users with their posted text and a new anonymous post, we aim to predict the most plausible author of this new post $q=\{w_{q,1}, w_{q,2},..., w_{q,T}\}$ from these users. In previous work, such as \cite{shrestha2017convolutional}, train a classification model taking a post as input and predicting the most plausible user given a set of candidates. In this paper, different from previous work, we train a post embedding model to learn the representation of a post and then compute a prediction function $\hat{y}_{u_i, q} = F(u_i, q|P_{u_i}, q, \theta)$, where $\hat{y}_{u_i, q}$ denotes the probability that the user $u_i$ tweeted this anonymous post $q$, and $\theta$ denotes the model parameters of learned post embedding model. 

\subsection{Post Embedding Module}
Figure~\ref{fig:framework_post_learning} illustrates the overall architecture of the post embedding module in our \textsf{DeepStyle} framework. The module learns the post embedding representations using triplet loss. Each triplet is formed by first randomly sampling an anchor post $p_{u,i}$ and a positive post $p_{u,j}$ that belongs to the same user $u$. We also randomly sample a negative post $p_{v,k}$, which is a post belonging to another user $v$.  With a set of triplets of posts, we learn the post embeddings using \textit{Multi-Style Post Representation}. In this \textit{Multi-Style Post Representation} scheme, we first perform data pre-possessing to extract different types of feature embeddings (e.g., word, character, bigram, POS tags) for each post among the triplets. These feature embeddings will be used as input for a set of Convolution Neural Networks (CNNs) to process and output latent representations of the individual features. Subsequently, a fusion function is used to combine the latent representations and output a post embedding. Finally the three post embeddings, $e_{u,i}$, $e_{u,j}$, and $e_{v,k}$, will be optimized using the triplet loss objective function.       

\begin{figure}[t]
    \centering
    \includegraphics[width=\textwidth]{framework_aa_2.pdf}
    \caption{Post embedding module of the \textsf{DeepStyle} framework}
    \label{fig:framework_post_learning}
\end{figure}

%Figure~\ref{fig:framework_post_learning} illustrates the overall architecture of our \textsf{DeepStyle} model, which consists of three main components: 1) input layer, which preprocesses the text of a post to generate multi-level sequences, i.e., lexical, character n-gram and POS tag. And then it parameterizes each token of the multi-level sequences as a vector using multi-level embedding matrices; 2) multi-level convolutional layer, which extracts the multi-level representations based on the multi-level embeddings using convolution operator and max-over-time pooling\cite{collobert2011natural}; 3) fusion layer: which fuses the multi-level representations of a post and generate the final representation of the post. 

\textbf{Feature Embeddings Extraction.} Previous studies have extensively explored the different types of features, such as words, characters, n-grams, syntactic, and semantic information for AA, \cite{stamatatos2009survey,ding2017learning,sari2018topic}. We leverage on the insights from previous studies to extract the following types of feature embeddings to represent a post $p_{u,i}$, $p_{u,j}$ or $p_{v,k}$. For simplicity, we use $p_{v,k}$ as an example.

% \begin{itemize}
%     \item \textit{Word}. A post $p$ is treated as a word token sequence. This word token sequence is then projected into a sequence of embedding representations, $x^w_{p,1}, \cdots, x^w_{p,l_{p,w}}$ where $l_{p,w}$ denotes the word token sequence length.
%     \item \textit{Character}. A post $p$ is treated as a character sequence and is also projected into a sequence of embedding representations, $x^c_{p,1}, \cdots, x^c_{p,l_{p,c}}$ where $l_{p,c}$ denotes the character sequence length.
%     \item \textit{Bi-gram}. Bi-gram has been identified to be one of the most useful features in AA \cite{shrestha2017convolutional}. We thus generate the character bi-grams for a given post $p$. The bi-grams sequence is then projected to its embedding representation, $x^b_{p,1}, \cdots, x^b_{p,l_{p,b}}$ where $l_{p,b}$ denotes the bi-gram sequence length.
%     \item \textit{POS Tag}. Part-of-speech (POS) tags contain morpho-syntactic information and are assigned to each word-token of a post $p$ based on contextual information. These POS tags capture the text expression style of users. We generate the POS tag sequence of $p$ using Stanford CoreNLP \cite{manning-EtAl:2014:P14-5} and project the POS tag sequence into its embedding representation $x^t_{p,1}, \cdots, x^t_{p,l_{p,t}}$ where $l_{p,t}$ denotes the POS tag sequence length.
% \end{itemize}

%\subsubsection{Input Layer}
%Previous studies on AA \cite{stamatatos2009survey,ding2017learning,sari2018topic} discussed the function of taxonomies of features, such as bag-of-words, word, character n-gram, syntactic and semantic information, and so on. Some papers \cite{shrestha2017convolutional,sapkota2015not} regard character n-grams as the most successful feature in AA. And \cite{shrestha2017convolutional} only uses the character n-grams as the input of its model. However, Word-level, syntactic, and semantic information can also play a significant effect on the accuracy of AA. The proposed model adopts multi-level information such as lexicon, character, character n-grams and POS tag as features to discover discriminative user style, and empirically verify the function of different features in table \ref{3} in the experiment section. In the following, for a post $p=\{w_1, w_2, ..., w_{T}\}$, we present the four sorts of feature extraction methods in detail.

%\textbf{Lexicon:} extracted in the post considers a text as a sequence of word-tokens. Obviously, different users have different habits of word usage. Besides, an important advantage of lexical feature is that it can be used in almost all languages with a corresponding tokenizer tool. We utilize a tokenizer to generator the word token sequence of a post and project each word token into its embedding representation: $P_{lex}=\{e_{lex,1}, e_{lex,2}, ..., e_{lex,T_l}\}$ via the lexical embedding matrix $E_{lex}$. Here, $e_{lex,j}\in R^d$ is the embedding vector for word token at the j-th position, and $d$ is the embedding size, and $T_l$ is the length of word tokens.

%\textbf{Character N-grams:} has been in identified as the most useful feature in AA. One hypothesis mentioned by \cite{shrestha2017convolutional} is that character n-grams features include much information, such as lexical content, syntactic content, means of punctuation,  and white space. Considering the efficiency of computing, we only generate character 2-grams from post text and project each 2-gram into a vector: $P_{ng}=\{e_{ng,1}, e_{ng,2}, ..., e_{ng,T_{ng}}\}$ via the character 2-gram embedding matrix $E_{ng}$.

%\textbf{Character:} has a significant advantage comparing to character n-grams. That is, the number of different characters is very small while character n-grams is extremely large. Combined with convolution operators based on multiple sizes of  kernels (such as 3, 4, 5), character level form can demonstrate the ability to capture local (3, 4, 5)-grams information without considering extensive vocabulary dictionary. We generate the character sequence of a post and project them into their embedding representations: $P_{ch}=\{e_{ch,1}, e_{ch,2}, ..., e_{ch,T_{ch}}\}$ via the character embedding matrix $E_{ch}$.

%\textbf{POS Tag:} containing morpho-syntactic information is assigned to each word-token based on contextual information. The level of POS tag also denotes different habits of text expression of users. we generate the POS tag sequence of post text with stanford corenlp \cite{manning-EtAl:2014:P14-5} and project each tag into its embedding representation: $P_{pos}=\{e_{pos,1}, e_{pos,2}, ..., e_{pos,T_{pos}}\}$ via the POS tag embedding matrix $E_{pos}$.

%Through the input layer, we can get multiple level embedding vectors of post text. It's worthy to note that we don't use the semantic information such as dependencies tree as a part of the proposed model's features. Although the content and structure of dependencies parsing contain much useful information on users' posts, there is difficult to utilize them. We are going to explore it in future work.

% The various types of extracted feature embeddings are used as input to the neural network layers to learn their latent representations, $e^w_p$, $e^c_p$, $e^b_p$, and $e^t_p$.  

%Through the input layer, we can get multiple level embedding vectors of post text. It's worthy to note that we don't use the semantic information such as dependencies tree as a part of the proposed model's features. Although the content and structure of dependencies parsing contain much useful information on users' posts, there is difficult to utilize them. We are going to explore it in future work.

%\subsubsection{Multi-level Convolutional Layer}
%overview: After xx, we obtain.  then implement xx. First, a convolutional module, then a full-connect. For simplicity, we use xxx. 

% \textbf{Neural Network Layers.} As shown in Figure~\ref{fig:framework_post_learning}, each input feature embedding sequence is processed by a separate neural network model. We use Convolutional Neural Network (CNN) to learn the latent representations of the input feature embeddings as previous hate-speech detection studies have shown that CNN outperforms sequence models (e.g., LSTM) in extracting such features from text \cite{DBLP:journals/corr/RuderGB16c,shrestha2017convolutional}. For example, a CNN is used to map the a post's word embedding sequence, $x^w_{p,1}, \cdots, x^w_{p,l_{p,w}}$ to $e^w$. In the following discussion, we shall ignore the superscript for simplicity. We first let $x_{p,i} \in R^d$ be token vector corresponding to $i$-th position in the input sequence of CNN, where $d$ is the dimension of the token vector. We unify the lengths of different input sequences to $l$. Input sequences longer than $l$ are pruned while shorter are padded. The input sequence is represented as follows:
% %    \vspace{-5px}
% \begin{equation}
%     x_{p,1:l} = x_{p,1} \oplus x_{p,2}\oplus...\oplus x_{p,l},
% \end{equation}
% %    \vspace{-1px}
% where $\oplus$ is the concatenation operator and $x_{p,1:l} \in \mathbb{R}^{l \times d}$ can be regarded as input matrix for CNN. A generic CNN function with $k_o$ filters is denoted as:
% % A generic CNN function with $k$ filters $H\in \mathbb{R}^{h\times d}$ is denoted as: 
% \begin{equation}
%     e_p = CNN(x_{p,1:l})
% \end{equation}
% Where $e_p\in \mathbb{R}^{k_o}$ is the final compact representation of the token sequence $x_{p,1:l}$.


% As illustrated in Figure 1, the multi-layer convolutional layer contains four CNN modules to process four different embedding representations from the input layer,  respectively. More explicitly, one CNN module is used to extract feature over word representation; one is over character 2-gram representation; one is over character representation, and the last one is over POS tag representation. 

% For the sake of description, we first introduce the working mechanism of CNN module regardless of different symbols for these four CNNs. We adopt a CNN structure similar to the model proposed in \cite{shrestha2017convolutional}. We let $x_i\in R^d$ be the token vector corresponding to $i$-th position in the input sequence of CNN. We unify the lengths of input sequences to $l$. Input sequences longer than $l$ are pruned while shorter are padded. That is, the input sequence is represented as:
% \begin{equation}
%     x_{1:l} = x_1\oplus x_2\oplus...\oplus x_l,
% \end{equation}
% where $\oplus$ is the concatenation operator. A generic CNN function with $k$ filters $H\in R^{h\times d}$ is denoted as: 
% \begin{equation}
%     v = CNN(x_{1:l})
% \end{equation}
% Where $v\in R^{d_a}$ is the final compact representation of a token sequence.

% More specifically, the convolution layer is composed of two stages: \textit{convolution} and \textit{pooling}. The convolution stage applies a set of $k$ convolution filters to the input sequence $x$. Each convolution filter $F \in \mathbb{R}^{h\times d}$ is applied to a window of $h$ input embedding vectors $x_{p,i:i+h-1}$ to produce a new feature scalar $c_i$ as follows:
% \begin{equation}
%     c_i = f(Fx_{p,i:i+h-1}+b),
% \end{equation}
% Where $b\in \mathbb{R}$ is a scalar bias term and $f$ is a non-linear function such as $tanh$ or $ReLU$. The filter $F$ is applied to each window of tokens in the embedding sequence to produce a feature map $c = \{c_1, c_2, ..., c_{l-h+1}\}$, where $c\in \mathbb{R}^{l-h+1}$. With $k_o$ filters, the first stage produces $k_o$ feature maps. 

% The next stage, pooling, adopts a max-over-time pooling operation. it is applied to each feature map and the maximum value $\hat{c} = \max\{c\}$ is taken as the feature corresponding to this particular filter. As a result, $k_o$ features are extracted from the feature maps to form the output of the CNN layer $e=\{\hat{c}_1, \hat{c}_2, ..., \hat{c}_{k_o}\}$. 

For the four types of input embeddings $\{x^w_{v,k}, x^c_{v,k}, x^b_{v,k}, x^t_{v,k}\}$, we obtain four types of output latent representations through multi-level CNN layer , i.e., word latent representation $e^w_{v,k}$, character latent representation $e^c_{v,k}$, bi-gram latent representation $e^b_{v,k}$, and POS tag latent representation $e^t_{v,k}$.

\textbf{Post Features Fusion Function.} After learning the latent representations of the various types of feature embeddings, we use a fusion function to combine the various latent representations of a post:
\begin{equation}
    e_{v,k} = Fuse(e^w_{v,k}, e^c_{v,k}, e^b_{v,k}, e^t_{v,k})
\end{equation}
where $Fuse(\cdot)$ is a typical fusion kernel, and $e_{v,k}$ has the same dimension as the input latent representations. In our proposed framework, we explore five different implementations the of $Fuse(\cdot)$: \textit{Mean}, \textit{Max}, \textit{Multilayer perceptron (MLP)}, \textit{Attention}\cite{DBLP:conf/naacl/YangYDHSH16}, and \textit{Capsule} \cite{sabour2017dynamic}.
% \begin{itemize}
%     \item \textit{Mean}. The mean operator, where we take the element-wise mean of the latent input representations:
%     \begin{equation}
%         e^{mean}_{v,k} = Mean(e^w_{v,k}, e^c_{v,k}, e^b_{v,k}, e^t_{v,k})
%     \end{equation}
%     \item \textit{Max}. Similar to mean fusion, we apply the max operator by taking the element-wise max value of the input latent representations:
%     \begin{equation}
%         e^{max}_{v,k} = Max(e^w_{v,k}, e^c_{v,k}, e^b_{v,k}, e^t_{v,k})
%     \end{equation}
%     \item \textit{Multilayer perceptron (MLP)}. We apply a MLP layer to concatenate the input latent representations, followed by a project matrix and a nonlinear transformation:
% %    \vspace{-5px}
%     \begin{equation}
%         e^{mlp}_{v,k} = \sigma(W_1^T(e^w_{v,k}\oplus e^c_{v,k}\oplus e^b_{v,k}\oplus e^t_{v,k}))
%     \end{equation}
%     where $\oplus$ is the concatenation operation, and $W_l\in R^{4d_a\times d_a}$ is a learnable weight. 
%     \item \textit{Attention}. The attention mechanism is proven to be a useful technique in NLP applications \cite{DBLP:conf/naacl/YangYDHSH16}. We apply an attention layer to measures the importance of the the various latent representations using the similarity of the vectors $e^g_{v,k}, g\in G=\{w, c, b, t\}$,  with a sentinel learning vector $u_w$:
% %    \vspace{-5px}
%     \begin{equation}
%         e^{att}_{v,k} = \sum_{g}a_g e^g_{v,k} 
%     \end{equation}
% %    \vspace{-1px}
%     \begin{equation}
%         a_g = \frac{\exp{u^T_g u_w}}{\sum_{i\in G} \exp{u^T_i u_w}}
%     \end{equation}
%     \begin{equation}
%         u_g = \mathrm{tanh}(W_a e^g_{v,k}+b_a)
%     \end{equation}

%     \item \textit{Capsule}. This mechanism iteratively updates the weight which denotes the similarity between input vectors and the output vector by the routing agreement algorithm \cite{sabour2017dynamic}. The output representation is defined by:
% %        \vspace{-5px}
%   \begin{equation}
%   \label{eqn:cap1}
%       e^{cap}_{v,k} = \mathrm{squash}(\phi) = \frac{\parallel \phi \parallel^2}{1+\parallel \phi \parallel^2} \frac{\phi}{\parallel \phi \parallel}
%   \end{equation}
% %       \vspace{-10px}
%     \begin{equation}
%     \label{eqn:cap2}
%         \phi = \sum_g c^{g}e^g_{v,k} 
%     \end{equation}
%     where squash() is a non-linear function, and $c_{g}$ is the coefficient indicating the importance of the latent representation $e^g_{v,k}$. Algorithm \ref{algo:routing} shows  the routing agreement. 
% \end{itemize}

% \begin{algorithm}[t]
%     \caption{Dynamic routing algorithm}
%     \label{algo:routing}
%     \begin{algorithmic}[1] 
%         \Function{Routing}{$e^g_{v,k}$, $iter$}
%             \STATE $\beta^g \gets 0$
%             \FOR{$iter$ iterations}
%             \STATE $c^g \gets \mathrm{softmax}(\beta^g)$ 
%             \STATE $\phi \gets \sum_g c^{g}e^g_{v,k} $
%             \STATE $e^{cap}_{v,k} = \mathrm{squash}(\phi)$
%                 \FOR {$g\in \{w, c, b, t\}$}
%                 \STATE $\beta^g \gets \beta^g + e^g_{v,k}*e^{cap}_{v,k}$
%                 \ENDFOR
%             \ENDFOR
%             \RETURN{$e^{cap}_{v,k}$}
%         %\EndFunction
%     \end{algorithmic}
% \end{algorithm}

% The fusion methods have an impact on our model's performance, and we will evaluate the performances of these post features fusion methods in our experimental evaluation.

%\subsubsection{Fusion Layer}
%With four compact representations $v_{lex}$, $v_{ng}$, $v_{ch}$ and $v_{pos}$ derived, a particular fusion unit has been adopted to combine these four features:
%\begin{equation}
%    r = Fuse(v_{lex}, v_{ng}, v_{ch}, v_{pos})
%\end{equation}
%where $Fuse(\cdot, \cdot, \cdot, \cdot)$ is a typical fusion kernel, and $r$ has the same dimension as $v$. We implement $Fuse(\cdot, \cdot, \cdot, \cdot)$ using five types of fusion:
%\begin{itemize}
%    \item \textit{Mean Fusion} is the mean operator, where we simply take the element-wise mean of the four vectors, as follows:
%    \begin{equation}
%        r_{mean} = MEAN(v_{lex}, v_{ng}, v_{ch}, v_{pos})
%    \end{equation}
%    \item \textit{Max Fusion} is similar to mean fusion, where we take the element-wise max operetor of the four representations:
%    \begin{equation}
%        r_{max} = MAX(v_{lex}, v_{ng}, v_{ch}, v_{pos})
%    \end{equation}
%    \item \textit{MLP Fusion} concatenates these four representations, followed by a project matrix and a nonlinear transformation:
%    \begin{equation}
%        r_{mlp} = \sigma(W_1^T(v_{lex}\oplus %v_{ng}\oplus v_{ch}\oplus v_{pos}))
%    \end{equation}
%    where $\oplus$ is the concatenation operator, $W_l\in R^{4d_a\times d_a}$ is the learning weight. 
%    \item \textit{Guard Attention} measures the important of the four different representations as the similarity of the vector $v_t, t\in \{lex, ng, ch, pos\}$  with a sentinel learning vector $u_w$ followed by:
    
%    \begin{equation}
%        r_{att} = \sum_{t}a_t v_t 
%    \end{equation}
%    \begin{equation}
%        a_t = \frac{\exp{u^T_t u_w}}{\sum_i %\exp{u^T_i u_w}} 
%    \end{equation}
%    \begin{equation}
%        u_t = \mathrm{tanh}(W_a v_t+b_a)
%    \end{equation}

%    \item \textit{Capsule Fusion} is iteratively updating the weight denoting the similarity between input vectors and the output vector by the routing agreement algorithm\cite{sabour2017dynamic}. The output capsule representation is computed by:
    
%  \begin{equation}
%       r_{cap} = \mathrm{squash}(s) = \frac{\parallel s \parallel^2}{1+\parallel s \parallel^2}\frac{s}{\parallel s \parallel}
%   \end{equation}
%    \begin{equation}
%        s = \sum_t c_{t}v_t 
%    \end{equation}
%    where "squash" is a non-linear function, and $c_{t}$ is the coefficient indicating the importance of the vector $v_t$. The routing by agreement is showed in Algorithm ?.
%\end{itemize}



% \begin{algorithm}
%     \caption{dynamic routing algorithm}
%     \begin{algorithmic}[1] 
%         \Function {Routing}{$Array, left, right$}
%             \State $result \gets 0$
%             \If {$left < right$}
%                 \State $middle \gets (left + right) / 2$
%                 \State $result \gets result +$ \Call{MergerSort}{$Array, left, middle$}
%                 \State $result \gets result +$ \Call{MergerSort}{$Array, middle, right$}
%                 \State $result \gets result +$ \Call{Merger}{$Array,left,middle,right$}
%             \EndIf
%             \State \Return{$result$}
%         \EndFunction
%     \end{algorithmic}
% \end{algorithm}

\subsection{User Style Aggregation Module}

A user publishes multiple posts on social media platforms. Each post contains some information that defines the user's writing style, which ultimately would help in authorship attribution. There are multiple ways to combine the post embeddings of a user $v$ to form the final user style embedding representation, $S_v$. In this paper, we introduce three types of aggregators for learning the post embedding of a user: \textit{Mean}, \textit{Max}, and \textit{Capsule} \cite{sabour2017dynamic}.
%For a user, there are many posts released. Each of these probably contains some information denoting this user's authorship attribution to some degree. Representation of a user is bound up with its released posts. However, A post or a handful of posts are difficult to represent a user. To differentiate different users more, we apply a particular aggregation function to aggregate the post embeddings of a single user into its style embedding. To avoid training again during inference period, we implement three types of non-training aggregators $agg: R^{M_u\times k_o} \rightarrow R^{k_o}$:
% \begin{enumerate}
%     \item \textit{Mean}. Takes the element-wise mean of a user's post embeddings:
%     \begin{equation}
%          S_v^{mean} = \frac{1}{M_v}\sum^{M_v}_{k}{e_{v, k}}  
%     \end{equation} 
%     \item \textit{Max}. Takes the element-wise max operator of a user's post embeddings.
%     \item \textit{Capsule}. Takes all the post embeddings as input capsules and use one output capsule to generate the final user style representation. The computation for this aggregator is similar to \ref{eqn:cap1} and \ref{eqn:cap2}, replacing the input with post embeddings. 
%     \begin{equation}
%         S_v^{cap} = squash(\phi_v) = \frac{\parallel \phi_v \parallel^2}{1+\parallel \phi_v \parallel^2}\frac{\phi_v}{\parallel \phi_v \parallel}
%     \end{equation}
%     \begin{equation}
%         \phi_v = \sum^{M_v}_{k} c_{v, k}e_{v,k} 
%     \end{equation}
%     where $squash()$ is a non-linear function, and $C_{v,k}$ is the coefficient indicating the importance of the post $e_{v,k}$.
% \end{enumerate}

Using the above three aggregators, we aggregated the users' post embeddings to form the user style embeddings, $S=\{s_1,s_2,...,s_N\}$. The user style embeddings will be be used to perform AA. We will further evaluate the three aggregation methods in our experiments.

%We generate style embedding for every user after the aggregation operator. while testing, we extract the query post representation by the trained post embedding module, then, calculate and rank the similarity of query post and all user style embeddings. The top1 user is the most plausible author we predict of the query post.  We will evaluate the three aggregation methods in experiments.

%\subsection{Optimization}
%Intuitively, we want two posts published by the same users, i.e., $p_{u,i}$ and $p_{u,j}$, to be close in the embedding space while posts from different users, i.e., $p_{u,i}$ and $p_{v, k}$, should be far apart. Thus, we aim to achieve the following:
%\begin{equation}
%    sim(e_{u,i}, e_{u,j}) > sim(e_{u,i}, e_{v,k}) + \gamma
%\end{equation}
%where $sim(\cdot)$ is a cosine similarity function (other similarity functions could be used), $e_{u,i}$, $e_{u,j}$ and $e_{v,k}$ are the representations of posts $p_{u,i}$, $p_{u,j}$ and $p_{v,k}$ respectively. $\gamma$ is a margin that is enforced between positive and negative pairs.

%We model this characteristics using the Triplet Loss function \cite{cheng2016person}:
%\begin{equation}
%    L = max(0, \gamma - sim(e_{u,i}, e_{u,j})+ sim(e_{u,i}, e_{v,k}))
%\end{equation}

% \subsection{Implementation Details}
% We optimize hyperparameters of our \textsf{DeepStyle} configurations on the development set of the Twitter 50-user subset without any task-specific fine-tuning. In the input layer, We set the same embedding size $d = 300$ for different style vocabularies. Additionally, we have added a dropout layer with $30\%$ dropout after the embedding layer for regularization. We have four CNN layers with the same structure to extract different style features in a multi-style post representation module. Each CNN layer has three filter windows of $3,4,5$ with 500 filters each. We set the margin $\gamma=0.01$ in the triplet loss to optimize the similarity of different posts and mini-batch size of 200 for faster training. We employ Adaptive Moment Estimation \cite{DBLP:journals/corr/KingmaB14} with a learning rate of $0.001$ to train our model. 

==> APWEB20 - DeepStyle (Cam-Ready)/related.tex <==
Authorship attribution (AA) is a widely studied research topic. Traditionally, feature engineering approaches were used to derive textual-related features from long documents such as emails and news articles. Subsequently, these derived features are used to train a classifier to identify an input document's owner \cite{koppel2009computational,stamatatos2009survey}. Commonly used features in AA includes character n-grams \cite{layton2010authorship,koppel2014determining,sapkota2015not,schwartz2013authorship}, lexical features, syntactical features, and document topics \cite{sundararajan2018represents,sari2018topic}. There are also recent studies that explore various deep learning approaches for AA. %Rhodes et al. \cite{rhodes2015author} applied Convolutional Neural Network (CNN) with word-level representation for AA. However, the study only applied deep learning approaches to perform AA on larger textual documents and evaluated on social media content.
 
In recent years, the AA task has been studied in the social media context. A comprehensive survey \cite{rocha2016authorship} provides an overview of AA methods for social media content. The short social media content poses some challenges to the traditional AA methods, \cite{koppel2014determining,shrestha2017convolutional}. To overcome the short text challenge, the existing methods aggregate multiple social media posts of a user into a single document and before applying the AA methods, \cite{layton2010authorship,ding2017learning}. Such an approach cannot adequately handle queries at the single social media post level. Shrestha et al. \cite{shrestha2017convolutional} attempted to overcome this challenge by performing AA using a CNN model with character n-gram features. The n-gram CNN model considers each short text post of a user as input to train a CNN model for AA. In similar studies, Ruder et al. \cite{DBLP:journals/corr/RuderGB16c} investigated the use of CNN with various types of word and character level features for AA, while Boenningoff et al. \cite{Boenninghoff2019} proposed a hybrid CNN-LSTM on word level features to perform AA. Although these works achieved reasonably good accuracy for AA in social media, they had utilized single input feature types to represent the users' posts used in training the deep neural network classifier and offer limited explainability. In this work, we address the limitations of the state-of-the-art by proposing \textsf{DeepStyle}, an embedding-based framework that learns the user style embedding representations using multiple types of features derived from posts to perform AA.

%Firstly, both works have only utilized single input feature types to represent the users' posts used in training the deep neural network classifier. Secondly, the existing works offer limited explainability on factors contributing to the AA results. Although \cite{shrestha2017convolutional} had conducted salient pattern analysis of the posts classified using the n-gram CNN model, they did not provide many insights of features that define a user's writing styles which subsequently help to perform AA correctly.  

 %Empirical analyses will also be conducted on user style embeddings to understand the features which define the writing style of users. 
